Machine-Made Media: Monitoring the Mobilization of Machine-Generated Articles on Misinformation and Mainstream News Websites

As large language models (LLMs) like ChatGPT have gained traction, an increasing number of news websites have begun utilizing them to generate articles. However, not only can these language models produce factually inaccurate articles on reputable websites but disreputable news sites can utilize LLMs to mass produce misinformation. To begin to understand this phenomenon, we present one of the first large-scale studies of the prevalence of synthetic articles within online news media. To do this, we train a DeBERTa-based synthetic news detector and classify over 15.46 million articles from 3,074 misinformation and mainstream news websites. We find that between January 1, 2022, and May 1, 2023, the relative number of synthetic news articles increased by 57.3% on mainstream websites while increasing by 474% on misinformation sites. We find that this increase is largely driven by smaller less popular websites. Analyzing the impact of the release of ChatGPT using an interrupted-time-series, we show that while its release resulted in a marked increase in synthetic articles on small sites as well as misinformation news websites, there was not a corresponding increase on large mainstream news websites.

==> canned.tex <==
BERT-Large \\
BERT-Large + Adv \\
BERT-Large + Adv + Para \\

RoBERTa-Large & 0.818 &0.997 & 0.985 & 0.868 & 0.919 \\
RoBERTa-Large + Adv \\
RoBERTa-Large + Adv + Para \\

DeBERTa-Large \\
DeBERTa-Large + Adv\\
DeBERTa-Large + Adv + Para\\



begin{table*}
\centering
%\tiny
\fontsize{8.0pt}{10pt}
\selectfont
\begin{tabular}{l|rrrrrrrr}
Model & Turing Benchmark & GPT-3.5 & GPT-3.5 w/ Adv & GPT-3.5 w/ Para & Article Forger & AI Writer &  Avg. \\ \midrule
\
OpenAI Roberta & &0.717/0.997/0.560 &0.159/0.442/0.097 &0.079/0.274/0.046 & 0.309/0.627/0.205 & 0.888/1.0/0.798 & 0.748/1.0/0.598\\
BERT & 0.790 & 0.996 & 0.981 & 0.922 &  0.947 & 0.927\\
BERT + Adv& 0.764 &  0.996 &0.979 & 0.938 & 0.939 &  0.923 \\
BERT+ Adv+Para &  0.801 & 0.996 & 0.971 & 0.955 &  0.970 & 0.939 \\
RoBERTa & 0.858 & 0.996 & 0.981 & 0.785 &  0.924 & 0.909 \\
RoBERTa + Adv & 0.832 & 0.996 & 0.985 & 0.917 & 0.988 & 0.944 \\
RoBERTa + Adv + Para & 0.838 & 0.994 & 0.986 & 0.902 & 0.992 & 0.942 \\
DeBERTa & 0.800 & 0.998 & 0.988 &0.810  &  0.921 & 0.903 \\
DeBERTa + Adv &  0.838 & 0.997 & 0.988 &  0.844 & 0.990 & 0.931\\
DeBERTa + Para &  0.838 & 0.997 & 0.988 &  0.844 & 0.990 & 0.931\\
DeBERTa + Adv + Para &0.847 & 0.998 &0.989 & 0.896 & 0.994 & 0.945\\




%0.452/1.0/0.292
\end{tabular}
\caption{\label{tab:benchmark} F1-Score/Precision/Recall of models on various benchmarks. } 
\vspace{-5pt}
\end{table*}


%(2) design a transformer-based classifier to identify machine-generated/synthetic articles across these different news websites, and (3) evaluate the aggregate level of engagement instance of these synthetic articles on the social media website Reddit. In this section, we give an overview of our collected datasets as well as details on how we trained and evaluated our system for identifying synthetic articles. 

%\subsection{News Collection and Reddit Dataset}
%To begin, we first outline the dataset of news websites and Reddit submissions that we collected in order to measure the presence and influence of machine-generated/synthetic content.

\begin{table}
\centering
\fontsize{8.5pt}{8}
\selectfont
\setlength\tabcolsep{4pt}
%\small
\begin{tabular}{l|ll}
 &  Misinfo Abs. \%  & Main. Abs.\% \\
 Rank &   Increase & Increase \\ \toprule
\textbf{All}  &+$10.17\%$ & +$9.18\%$\\ \midrule
Rank $<$ 10K & +$6.26\%$ & +$5.79\%$\\ 
10K $<$ Rank $<100$K  & +$10.83\%$ & +$5.86\%$\\ 
100K $<$ Rank $<1$M  & +$8.20\%$ & +$6.61\%$\\ 
1M $<$ Rank $<10$M  & +$12.48\%$ & +$11.51\%$\\ 
Rank $>10$M  & +$13.08\%$ & +$16.45\%$\\ 
\bottomrule
\end{tabular}
\caption{\label{tab:largest-percentage} Total absolute percentage increase in machine-generated/synthetic articles between January 2022, and April 1, 2023.} 
\vspace{-10pt}
\end{table}



\begin{table}
\centering
\footnotesize
\begin{tabular}{l|rl}
%\toprule
\textbf{Subreddit}&  \textbf{\% Synthetic} & \textbf{Top Synthetic Domain} \\\midrule
r/bad\_cop\_no\_donut & 33.1\% & kwtx.com  \\
r/politics  & 14.7\% & thehill.com\\
r/conservatives  & 10.3\%  & ustthenews.com\\
r/politicaldiscussion & 8.5\% & cnn.com\\
r/conspiracy & 6.7\% & independent.co.uk \\
\bottomrule

\end{tabular}
\caption{\label{tab:test-dataset} Political Subreddits (with at least 25 articles posted from within our dataset) with the highest percentage of synthetic articles.} 
\vspace{-10pt}
\end{table}


\begin{table}
\centering
\footnotesize
\begin{tabular}{l|r}
%\toprule
\textbf{}&  \textbf{\% Cohen's D} \\\toprule
Mainstream &  1.09\\
Misinformation & 1.36\\
\bottomrule

\end{tabular}
\caption{\label{tab:test-dataset} Performing a pairwise comparison of submissions from individual domains that were human-written vs. machine-generated. Submissions featuring human-written articles on average, received more Reddit comments between January 2022 and March 2023, compared to machine-generated/synthetic articles. For both mainstream and misinformation the difference in the number of comments between machine-generated and human-written articles was \textbf{statistically significant} (\textit{i.e}, $p\approx0$). }
\vspace{-10pt}
\end{table}


\begin{figure*}
  \centering
  \includegraphics[width=0.90\linewidth]{LaTeX/figures/machine_gen_pipeline.drawio.png}


\caption{Pipeline for Classifying news articles as human-written or machine-generated/synthetic. }
\label{fig:pipeline}
\vspace{-5pt}
\end{figure*}

\begin{table}
\centering
\footnotesize
\begin{tabular}{l|rl}
%\toprule
\textbf{Subreddit}&  \textbf{\% Synthetic}  & \textbf{Top Synthetic Domain} \\\midrule
r/bscmoonshots & 71.4\% & benzinga.com  \\
r/cryptomoonshots  & 62.1\% & benzinga.com\\
r/cryptomars  & 53.8\% & benzinga.com  \\
r/czcalls & 46.0\%  & investopedia.com\\
r/reddevils & 43.0\%   & bbc.com\\
\bottomrule

\end{tabular}
\caption{\label{tab:subreddit-most-syn} Subreddits (with at least 25 articles posted from within our dataset) with the highest percentage of synthetic articles. Many of these subreddits focus on cryptocurrency, sports (Red Devils is a subreddit dedicated to the UK football team Manchester United), or stocks.} 
\vspace{-10pt}
\end{table}

\begin{table}
\centering
\fontsize{6.4pt}{8}
\selectfont
\setlength\tabcolsep{4pt}
\begin{tabular}{lrr|lrr}
\textbf{Misinfo}  &\textbf{Abs. \%}  &  \textbf{CrUX}& \textbf{Main.} &\textbf{Abs. \%} 
 &  \textbf{CrUX}\\
\textbf{Domain} & \textbf{Increase} & \textbf{Rank} & \textbf{Domain} & \textbf{Increase} & \textbf{Rank} \\ \toprule
foreignpolicyi.org & 54.9\% &$<$10M  & indexmundi.com & 71.6\% & $<$100K \\
radiopatriot.net & 53.0\%&$<$10M & truththeory.com & 58.3\% &$<$10M\\
thefrisky.com & 49.6\% &$<$1M & vladtv.com & 57.0\% & $<$100K \\
patriotnewsdaily.com &  46.1\% & $<$10M & marketwatch.com & 56.0\% & $<$10K \\
newsexaminer.net & 42.8\%& $<$10M  & the-daily.buzz & 50.7\%  &$<$10M\\
theunionjournal.com &  41.8\%& $<$10M  & digitaljournal.com & 46.6\% &$<$1M \\
bestnewshere.com & 38.0\% & $<$100K & theleoterrell.com & 50.0\% &$<$10M\\
legitgov.org & 36.8\% & $<$10M  & influencewatch.org & 43.1\% & $<$10M \\
redvoicemedia.com& 36.3\% &$<$1M & thelist.com & 41.7\%& $<$100K \\
newsblaze.com & 35.6\% & $<$10M & investing.com & 38.9\%  & $<$10K\\
\bottomrule
\end{tabular}
\caption{\label{tab:largest-percentage-increase} Misinformation and Mainstream Websites with the largest increase in machine-generated content between January 2022, and March 2023. } 
\end{table}


==> ethics-questionaire.tex <==
\subsection{Paper Checklist to be included in your paper}

\begin{enumerate}

\item For most authors...
\begin{enumerate}
    \item  Would answering this research question advance science without violating social contracts, such as violating privacy norms, perpetuating unfair profiling, exacerbating the socio-economic divide, or implying disrespect to societies or cultures?
   \answerYes{Yes, our work largely focuses on uncovering the rate of usage of synthetic articles. Our work does not invade the privacy of individuals, collects only public data, and does not focus on any particular culture.}
  \item Do your main claims in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{Yes. Our abstract is largely reflective of our work.}
   \item Do you clarify how the proposed methodological approach is appropriate for the claims made? 
    \answerYes{Yes. Given our need to understand the use of synthetic articles on news websites, we so through Section~\ref{sec:detect} how our methodology precisely identifies synthetic articles.}
   \item Do you clarify what are possible artifacts in the data used, given population-specific distributions?
    \answerYes{Yes, we note that specific data peculiar to given websites may be part of the data collected. We note that this data is all public, however and does not reveal the personal data on any given individual.}
  \item Did you describe the limitations of your work?
    \answerYes{Yes, and we detail them in the Discussion}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNo{No, we do not believe that there are any immediate negative social repercussions}
      \item Did you discuss any potential misuse of your work?
    \answerNo{No; our work seeks to detect synthetic articles at a large scale. While potentially our system could be utilized to overly penalize those that publish synthetic articles, we have noted in our work that we focus on trends in the use of synthetic articles, not on predicting whether any specific article is synthetic  }
    \item Did you describe steps taken to prevent or mitigate potential negative outcomes of the research, such as data and model documentation, data anonymization, responsible release, access control, and the reproducibility of findings?
    \answerYes{Yes, for the articles scraped we only release their URLs and not their texts. We also release our model to GitHub to allow for reproducibility  }
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{Yes and we have made sure that it is clear }
\end{enumerate}

\item Additionally, if your study involves hypotheses testing...
\begin{enumerate}
  \item Did you clearly state the assumptions underlying all theoretical results?
    \answerYes{Yes, and where appropriate we have interpreted what these results mean}
  \item Have you provided justifications for all theoretical results?
    \answerNA{NA}
  \item Did you discuss competing hypotheses or theories that might challenge or complement your theoretical results?
    \answerNA{NA}
  \item Have you considered alternative mechanisms or explanations that might account for the same outcomes observed in your study?
    \answerYes{Yes, in our limitations section, we discus several alternative explanations for our data.}
  \item Did you address potential biases or limitations in your theoretical framework?
    \answerYes{Yes, we addressed the potential biases and limitations of our classifier in Section~\ref{sec:dataset} }
  \item Have you related your theoretical results to the existing literature in social science?
    \answerYes{Yes, see Section~\ref{sec:related}}
  \item Did you discuss the implications of your theoretical results for policy, practice, or further research in the social science domain?
    \answerYes{Yes, we discussed how research should information future AI detection systems and discussed the need to understand the growth of websites that primarily publish synthetic data.}
\end{enumerate}

\item Additionally, if you are including theoretical proofs...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{NA}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{NA}
\end{enumerate}

\item Additionally, if you ran machine learning experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Yes, we have included a redacted GitHub link}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:detect}}
     \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Yes, we benchmark and test our models across multiple datasets to better give an indication of the robustness of our results. We further include error bars for our results}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:detect}}
     \item Do you justify how the proposed evaluation is sufficient and appropriate to the claims made? 
    \answerYes{Yes, we have outlined these details in Section~\ref{sec:detect}}
     \item Do you discuss what is ``the cost`` of misclassification and fault (in)tolerance?
   \answerYes{Yes, we have outlined these details in Section~\ref{sec:detect}}
  
\end{enumerate}

\item Additionally, if you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Yes, we have cited Pu et. al's work~\cite{pu2022deepfake}}
  \item Did you mention the license of the assets?
    \answerNA{NA}
  \item Did you include any new assets in the supplemental material or as a URL?
    \answerYes{Yes, we have included a redacted GitHub link to the URLs  used in this project}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Yes, we have cited Pu et. al's work~\cite{pu2022deepfake} and outlined how we have obtained data from them}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{NA}
\item If you are curating or releasing new datasets, did you discuss how you intend to make your datasets FAIR?
\answerYes{Yes, our dataset is findable, accessible, interoperable, and reusable as we post in on GitHub and it consists of a list of urls. }
\item If you are curating or releasing new datasets, did you create a Datasheet for the Dataset? 
\answerYes{Yes, we outline in our GitHub page which domains are included within our dataset, (the methodology for collection is listed in the paper), and we document how it is supposed to be used. We note that our dataset just consists of a list of URLs as we do not release the news article contents.}
\end{enumerate}

\item Additionally, if you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots?
    \answerNA{NA}
  \item Did you describe any potential participant risks, with mentions of Institutional Review Board (IRB) approvals?
    \answerNA{NA}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{NA}
   \item Did you discuss how data is stored, shared, and deidentified?
   \answerNA{NA}
\end{enumerate}

\end{enumerate}

==> topics-table.tex <==
\begin{table*}
\hspace{-20pt}
\begin{minipage}{.3\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{Jan. 2022, Rank $<$ 10K}}\\
\toprule
Misinfo. &    & Mainstream.     \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
zelensky, biden, dr, & 135& covid19, january, cases & 854 \\
djokovic, australia, novak & 132 & watchlist,nasdaq,s\&p, & 376 \\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{15pt}
\begin{minipage}{.3\textwidth}
\centering
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{4pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{Jan. 2022, 10K $<$ Rank $<100$K }}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
ukraine, russia, nato, & 434 &  commerical,kg, commodity &1,491 \\
lotto, win, number & 193 & yield, kg, cattle & 1,167 \\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{25pt}
\begin{minipage}{.3\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{4pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{Jan. 2022, 100K $<$ Rank $<1$M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
democrat, trump, republican, & 82  &  covid19,dashboard,sick & 613 \\
trump, january, capitol & 60 & price, watch, invest & 533  \\
\bottomrule
\end{tabular}
\end{minipage}

\begin{minipage}{.5\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{Jan. 2022, 1M $<$ Rank $<10$M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
covid, pfzier, american, & 59  & astrazeneca, pfizer, mild & 72\\
china, beijing, ccp & 36 & january, capitol, trump  & 42\\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{10pt}
\begin{minipage}{.5\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{Jan. 2022, Rank $>$ 10M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
covid19, dr, biden, & 101  & biden, trump, republican & 27\\
senate, republican, rep & 73 & bluetooth, bose, headphones  & 23\\
\bottomrule
\end{tabular}
\end{minipage}


\hspace{-20pt}
\begin{minipage}{.3\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{March 2023, Rank $<$ 10K}}\\
\toprule
Misinfo. &    & Mainstream.     \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
zelensky, kremlin, prigozhin, & 237& market, watch, stock & 2,229 \\
football, game, score & 231 & degree,murder, sentence & 1,193 \\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{28pt}
\begin{minipage}{.3\textwidth}
\centering
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{March 2023, 10K $<$ Rank $<100$K }}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
russia, ukraine, putin, & 298 &  suspect,custody, arrest &1,943 \\
biden, desantis, washington & 267 & corp, llc, nasdaq & 1,785 \\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{18pt}
\begin{minipage}{.3\textwidth}
\centering
%\scriptsize
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{March 2023, 100K $<$ Rank $<1$M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
trump, biden, fox, &277  &  murder, police, sentence & 3,003 \\
trump, fbi, bragg & 226 & ncaa, basketball, carolina & 2,670  \\
\bottomrule
\end{tabular}
\end{minipage}
%\hspace{7pt}

\begin{minipage}{.5\textwidth}
\centering
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{March 2023, 1M $<$ Rank $<10$M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
ukraine, russia,putin, & 201  & trump, manhattan, bragg & 213\\
trump, democrats, fbi & 159 & covid, uk, pfizer  & 208\\
\bottomrule
\end{tabular}
\end{minipage}
\hspace{10pt}
\begin{minipage}{.5\textwidth}
\centering
\fontsize{6.5pt}{5pt}
\setlength{\tabcolsep}{2pt}
\selectfont
\begin{tabular}{lrlr}
 \multicolumn{4}{c}{\textbf{March 2023, Rank $>$ 10M}}\\
\toprule
Misinfo. &    & Mainstream.  &    \\
Topics &  \# Art.   &Topics &   \# Art.\\ \midrule
craigslist, tinder, italian, & 107  & ncaa, basketball, game & 172\\
loan, payday, cash & 88 & trump, manhattan, fox  & 110\\
\bottomrule
\end{tabular}
\end{minipage}
\caption{\label{tab:topics-jan2022} The top synthetic topics in January 2022, and March 2023, among misinformation and mainstream news websites in every striation of popularity.}
\vspace{-15pt}
\end{table*}
